Boolean Unateness Testing with $\widetilde{O}(n^{3/4})$ Adaptive Queries

We give an adaptive algorithm which tests whether an unknown Boolean function $f\colon \{0, 1\}^n \to\{0, 1\}$ is unate, i.e. every variable of $f$ is either non-decreasing or non-increasing, or $\epsilon$-far from unate with one-sided error using $\widetilde{O}(n^{3/4}/\epsilon^2)$ queries. This improves on the best adaptive $O(n/\epsilon)$-query algorithm from Baleshzar, Chakrabarty, Pallavoor, Raskhodnikova and Seshadhri when $1/\epsilon \ll n^{1/4}$. Combined with the $\widetilde{\Omega}(n)$-query lower bound for non-adaptive algorithms with one-sided error of [CWX17, BCPRS17], we conclude that adaptivity helps for the testing of unateness with one-sided error. A crucial component of our algorithm is a new subroutine for finding bi-chromatic edges in the Boolean hypercube called adaptive edge search.

==> temp - Erik/appendices.tex <==
% !TEX root =  writeup.tex

\section{Proof of the persistency lemma}\label{persistency-proof}

We give a proof of Lemma \ref{persistency-lemma}, which is a slight modification of Lemma 9.3 of \cite{KMS15}.

\begin{lemma}[Persistency lemma]
For $\gamma\in(0,1]$ and $\tau\in[0,n]$, the fraction of $(\tau,\gamma)$-non-persistent points is at most $O(I_f\cdot \tau/(n\gamma))$.
\end{lemma}

\begin{proof}
Let $\eta$ be the fraction of $(\tau, \gamma)$-non-persistent points. Consider the following random process:
\begin{enumerate}
\item we draw $\bx\in\{0,1\}^n$ uniformly at random.\vspace{-0.12cm}
\item we flip $\tau$ bits from $\bx$ uniformly at random to get $\by \in \{0, 1\}^n$.
\end{enumerate}
Let $(\bx, \by) \sim \calD$ be the distribution supported on pairs $x, y \in \{0, 1\}^n$ given by the above procedure. Let $\calD_{x}$ be the distribution supported on $\{0, 1\}^n$ given by sampling $\by$ where $(\bx, \by) \sim \calD$ conditioned on $\bx = x$.
For each $x\in\{0,1\}^n$, let
\[ r_{x} =\begin{cases} \Prx_{\by \sim \calD_{x}}[f(x) \neq f(\by)] &  \text{if $x$ is $(\tau,\gamma)$-non-persistent} \\
							0 & \text{otherwise} \end{cases} \]

By definition, for $(\tau,\gamma)$-non-persistent points $x$ we have $r_x\geq \gamma$, which implies:

\[ \Prx_{(\bx, \by) \sim \calD}[f(\bx) \neq f(\by)] = \frac{1}{2^n} \sum_{x \in \{0, 1\}^n} \Prx_{\by \sim \calD_{x}}[f(x) \neq f(\by)] \geq \frac{1}{2^n} \sum_{x \in \{0, 1\}^n} r_{x} \geq \gamma \cdot \eta \]

On the other hand, consider the following random process:
\begin{enumerate}
\item We draw $\bx_0 \in \{0, 1\}^n$ uniformly at random.\vspace{-0.12cm}
\item For each $k \in [\tau]$,  pick a random coordinate $\bi \in [n]$ that has not been chosen and let $\bx_k = \bx_{k-1}^{(\bi)}$.
\end{enumerate}
Note that $(\bx_0, \bx_{\tau})$ is distributed as $\calD$. Additionally, we have
\[ \Prx_{(\bx, \by) \sim \calD}[f(\bx) \neq f(\by)] \leq \sum_{k=1}^{\tau} \Prx_{\bx_{k-1}, \bx_{k}}\left[f(\bx_{k-1}) \neq f(\bx_{k}) \right] \leq \tau \cdot \frac{I_f}{n}, \]
where in the last step, we used the fact that each $(\bx_{k-1}, \bx_{k})$ is distributed as a uniform edge of the hypercube.
Combining the two inequalities above, we obtain $\eta = O ( (I_f \cdot \tau)/{(n\cdot \gamma)} )$.
\end{proof}

\section{Unateness testing algorithm for high-influence functions}
\label{sec:high-inf}

We note that implicitly, Lemma 9.1 of \cite{KMS15} proves the following lemma:
\begin{lemma}\label{blabla1}
If $f \colon \{0, 1\}^n \to \{0, 1\}$ has $I_f > 6 \sqrt{n}$, then
\begin{equation}\label{lalahehe}
\frac{1}{2^n} \sum_{i=1}^n \min \big\{ |E_i^+|, |E_i^-| \big\} \geq 2 \sqrt{n}.
\end{equation}
\end{lemma}

In particular, it implies that if $I_f\ge 6\sqrt{n}$ then $f$ cannot be unate.
Next we slightly modify the algorithm of \cite{CS16b} to obtain the following lemma:
\begin{lemma}\label{blabla2}
There is an $ O\ ( \sqrt{n} \cdot \log^2(n) )$-query, non-adaptive algorithm that, given
  any function $f$ that satisfies (\ref{lalahehe}),
  finds an edge violation of $f$ to unateness with probability at least $2/3$.
%Let $f \colon \{0, 1\}^n \to \{0, 1\}$ satisfy
%\[ \frac{1}{2^n} \sum_{i=1}^n \min\{ |E_i^+|, |E_i^-| \} = \Omega(\sqrt{n}). \]
%Then, there exists an algorithm which finds a violation to unateness using
%many queries.
\end{lemma}

Lemma \ref{hehelem} follows by combining Lemma \ref{blabla1} and Lemma \ref{blabla2}. For completeness, we include the algorithm of \cite{CS16b} (with modified parameters) in order to prove Lemma~\ref{blabla2}.

\begin{figure}[t!]
\begin{framed}
\noindent \texttt{Unate-E-Tester}, the unateness tester from \cite{CS16b} which rejects functions satisfying (\ref{lalahehe}).
\vspace{-0.16cm}
\begin{flushleft}\noindent {\bf Input:} Query access to $f \colon \{0, 1\}^n \to \{0, 1\}$ satisfying (\ref{lalahehe}).

\noindent {\bf Output:}  Either ``unate,'' or two edges constituting an edge violation for $f$.

\begin{itemize}

\item[] \vskip -.02in \hspace{-0.2cm}Repeat the following for $r = 1, 2,\dots, L = \lceil \log(8n) \rceil$: \vspace{-0.08cm}

\begin{enumerate}

\item \vskip -.02in Repeat the following $s_r = \left\lceil \dfrac{20 \sqrt{n}\cdot \log(8n)}{2^r} \right\rceil$ times: 

\item  Sample a direction $\bi \sim [n]$ uniformly at random and sample $4 \cdot 2^r$ random edges in direction $\bi$ and query all end points. Return an edge violation if one is found.

\end{enumerate}
\item[] \vskip -0.045in \hspace{-0.2cm}If we have not found any violation in line 2, return ``unate.'' 
\end{itemize}
\end{flushleft}\vskip -0.14in
\end{framed}
\caption{Description of the \algsecond~for Case 2 of the algorithm.} \label{fig:case2}
\end{figure}

\begin{proof}[Proof of Lemma~\ref{blabla2}]
Let $\mu_i = \frac{\min\{|E_i^+|, |E_i^-|\}}{2^n}$. For any $r = [L]$, let $i \in S_r$ be the set of directions where 
\[ \frac{1}{2^r} \leq \mu_i \leq \frac{1}{2^{r-1}}. \]
If $\mu_i \leq \frac{1}{8n}$, then all such directions $i$ contribute at most $\frac{1}{8}$ to the RHS of (\ref{lalahehe}).
Thus, there exists one direction $r^*$ such that
\[ \frac{1}{2^n} \sum_{i \in S_{r^*}} \min\{ |E_i^+|, |E_i^-| \} \geq \frac{2\sqrt{n} - 1/8}{\log (8n)} \geq \frac{\sqrt{n}}{\log(8n)}, \]
and $|S_{r^*}| \geq \frac{2^{r^*} \sqrt{n}}{2\log(8n)}$. Thus, at the iteration corresponding to $r^*$ of \texttt{Unate-E-Tester}, the probability $\bi \in S_{r^*}$ is at least $\frac{2^{r^*}}{2\sqrt{n} \log(8n)}$. Conditioned on having sampled some $i \in S_{r^*}$, the probability that we do not observe an edge in $E_i^+$ in the first $2 \cdot 2^{r^*}$ edges is at most $(1 - \mu_i)^{2 \cdot 2^{r^*}} \leq e^{-2}$. Likewise, the probability we do not observe an edge in $E_i^-$ in the second $2 \cdot 2^{r^*}$ edges is at most $e^{-2}$, thus, with probability $1 - 2e^{-2} \geq \frac{7}{10}$, we observe an edge violation. 

Putting things together, the probability that we observe an edge violation in one iteration of line 2 with $r = r^*$ is at least $\frac{7 \cdot 2^{r^*}}{20 \cdot \sqrt{n} \log(8n)}$. Since we repeat line 2 for $s_r = \lceil \frac{20 \sqrt{n} \log (8n)}{2^{r^*}}\rceil$ times, we find an edge violation with high constant probability.
\end{proof}


\section{Overlap of two random sets of certain size}
\label{apphehe}

Let $k,\ell\in [n]$ be two positive integers with $\alpha=k\ell/n$.
We are interested in the size of $|\bS\cap \bT|$ where $\bS$ is a random $k$-sized subset of $[n]$
  and $\bT$ is a random $\ell$-sized subset of $[n]$, both drawn uniformly.

%\begin{lemma}\label{appendix1}
%If $\alpha \le \log^2 n$, then the probability of $|\bS\cap\bT|\ge 2\log^2 n$ is $\exp(-\Omega(\log^2 n))$.
%\end{lemma}
%\begin{proof}
%Let $k$ and $\ell$ be two positive integers with $k\ell\le n\log^2 n$.
%We show that if we draw a random $k$-sized set $\bS\subseteq [n]$ and
%  a random $\ell$-sized set $\bT\subseteq [n]$ independently and uniformly,
%  then the probability of $| \bS\cap \bT|\ge 2\log^2 n$ is at most $\exp(-\Omega(\log^2 n))$.
%(Note that in our applications one of the two sets is fixed and the other is drawn uniformly at random.
%By symmetry the probability is exactly the same as the case we study here with both sets drawn uniformly at random.)
%Let $\bX_i$ be the random variable that is $1$ if
%  the index we add to $\bT$ belongs to $\bS$ in the $i$th round and is $0$ otherwise.
%
%Using the Chernoff bound (together with a simple coupling argument), the probability of
%  $\sum \bX_i\ge 2\log^2n$ is at most $\exp(-\Omega(\log^2 n))$.
%\end{proof}

\begin{lemma}\label{appendix1}
%If $\alpha \ge \log^2 n$, then the probability of $|\bS\cap\bT|\ge  4\alpha$ is $\exp(-\Omega(\log^2 n))$.
For any $t\ge 4\alpha$, the probability of $|\bS\cap\bT|\ge  t$ is at most $\exp(-\Omega(t))$.
\end{lemma}
\begin{proof}
We assume without loss of generality that $k\ge \ell$.
If $\ell> n/2$, the claim is trivial as $\alpha> n/4$ and $t\ge 4\alpha> n$.
We assume $\ell\le n/2$ below.

We consider the following~process.
We draw $\bS$ first. Then we add random (and distinct) indices of $[n]$ to  $\bT$ round by round for $\ell$ rounds.
In each round we pick an index uniformly at random from those that
  have not been added to $\bT$ yet.
Clearly this process generates the same distribution of $\bS$ and $\bT$ that we are interested in.

%, and we consider the same random process.


For each $i\in [\ell]$, we let $\bX_i$ be the random variable that is set to $1$ if
  the index in the $i$th round belongs to $\bS$ and is $0$ otherwise.
Although $\bX_i$'s are not independent, the probability~of $\bX_i=1$ is at most
  $k/(n-\ell)\le 2k/n$ using $\ell\le n/2$,
  for any fixed values of $\bX_1,\ldots,\bX_{i-1}$.
%As a result, the probability of $\bX_i=1$ is at most
%  $k/(n-\ell)\le 2k/n$, using $\ell\le n/2$.
Thus, the expectation of $\sum_{i\in [\ell]} \bX_i$ is at most $2k\ell/n=2\alpha$.
The lemma follows directly from the Chernoff bound (together with a standard coupling argument).
\end{proof}


==> temp - Erik/intro.tex <==
% !TEX root =  writeup.tex

\section{Introduction}

A Boolean function $f \colon \{0, 1\}^n \to \{0, 1\}$ is \emph{monotone}
  if every variable of $f$ is non-decreasing, and is
  \emph{unate} if every variable of $f$ is either non-decreasing or non-increasing
  (or equivalently, there exists an $r\in \{0,1\}^n$ such that $g(x)=f(x\oplus r)$ is monotone,
  where $\oplus$ is the bit-wise XOR).~Both~problems of testing \emph{monotonicity}
  and \emph{unateness}
  were first introduced in \cite{GGLRS00}.
 %   as a natural extension of
 % testing \emph{monotonicity},
The goal is to design~an algorithm that decides whether
  an unknown $f:\{0,1\}^n\rightarrow \{0,1\}$ has the property being tested~or is far from having the property (see Section \ref{sec:preliminaries} for the formal definition) with as few queries as possible.
After a sequence~of developments from the past few years
  \cite{CS14, CST14, KMS15, CDST15, BB16, CS16, CWX17}, the query complexity of non-adaptive
  algorithms for monotonicity has been pinned down at $\smash{\widetilde{\Theta}(n^{1/2})}$;
  for adaptive monotonicity testing algorithms
  there remains a gap between $\widetilde{O}(n^{1/2})$
  and $\widetilde{\Omega}(n^{1/3})$. % for the query complexity of adaptive algorithms for monotonicity.
The query complexity of testing unateness, however, is less well-understood.
%  which has been a touchstone problem in property testing for more than fifteen years
%\cite{DGLRRS99, EKKRV00, FLNRRS02, F04, BKR04, AC06, ACCL07, HK08, RS09, BBM12, BCGM12, RRSW12, BRY14a, BRY14b, CS13, C14, CS14, CST14, KMS15, CDST15, BB15, BB16, CS16, CWX17}.

The seminal work of \cite{GGLRS00} presented an $O(n^{3/2}/\eps)$-query algorithm
  for testing unateness of Boolean functions.
%that tests whether an unknown Boolean function $f\colon \{0, 1\}^n \to \{0, 1\}$ is unate or $\eps$-far from every unate function.
It proceeds by sampling $O(n^{3/2}/\eps)$ \emph{edges}\footnote{A pair of points $(x,y)$ in
$\{0,1\}^n$ is
  an edge in the Boolean hypercube if $x_i\ne y_i$ at exactly one coordinate $i\in [n]$.
We will refer to $i$ as the direction~of $(x,y)$.
An edge $(x,y)$
  along direction $i$ is \emph{bi-chromatic}
  (in $f$) if $f(x)\ne f(y)$; it~is \emph{monotone} if it is bi-chromatic and has
  $f(x)=x_i$;
  %$x_i=0$, $y_i=1$ and $f(x)=0$ or $x_i=1$, $y_i=0$ and $f(x)=1$;
  it is \emph{anti-monotone} if it is bi-chromatic but not~monotone.}
  of $\{0,1\}^n$ uniformly at random, %, or pairs of points $x, x' \in \{0, 1\}^n$ which differ in one bit.
  and rejects only when it finds a so-called \emph{edge violation} ---
  %The hope is that when a function is $\eps$-far from unate, the algorithm will find an \emph{edge violation} ---
  two edges $(x, y)$ and $(x', y')$ in the same direction $i$ for some $i\in [n]$ such that
  one is monotone and the other is anti-monotone.~By definition %$f$ cannot be unate if such an edge violation exists.
%$x \leq x'$ and $y \leq y'$ where $f(x) < f(x')$, but $f(y) > f(y')$.
the existence of an edge violation ensures that the function is not unate~and thus,
  the algorithm has one-sided error (i.e., it always accepts a unate function); we refer to algorithms which always accept unate functions as \emph{one-sided}.
This algorithm is non-adaptive as well (i.e.,~all queries can be made at once).
For the correctness, \cite{GGLRS00} showed that after sampling $O(n^{3/2}/\eps)$ random edges an edge violation is found with high probability when $f$ is $\eps$-far from unate.
%, since in direction $i \in [n]$, $(x, x')$ is a \emph{monotone} edge and $(y, y')$ is an \emph{anti-monotone} edge.



%If the algorithm finds such a violation to unateness, the algorithm may safely output ``not-unate''. If an edge violation is never found, the algorithm outputs ``unate''. A simple observation is that this test is \emph{non-adaptive}, which means all queries may be made at once, as well as \emph{one-sided}, which means the algorithm always accepts unate functions.


Recently, \cite{KS16} obtained the first improvement to the upper bound of \cite{GGLRS00} by presenting an
  ${O}( n\log n/\eps)$-query  adaptive, one-sided algorithm.
% At a high level, they obtain a lower query complexity by using a binary search strategy: they first perform multiple instances of binary search to look for influential directions and finding bi-chromatic edges in these directions, and then perform a monotonicity tester choosing the direction of the partial order according to the edges observed.
Later, \cite{BMPR16} generalized the algorithm~to work for real-valued functions over the $n$-dimensional hypergrid, $f \colon [m]^n \to \R$.
% and \cite{CS16b}  showed
%  that almost the same~upper bound  (up to a polylogarithmic factor\hspace{0.03cm}\footnote{The query complexity of the algorithm
%    of \cite{KS16} is $O(n\log n/\eps)$ and that of \cite{CS16b} is $O(n\log(n/\eps)/\eps)$.}) of \cite{KS16} can be achieved using a non-adaptive, one-sided algorithm.
The current best upper~bounds for testing unateness of Boolean functions are $O((n/\eps)\log(n/\eps))$ for non-adaptive algorithms
  \cite{CS16b,BCPRS17}, and $O(n/\eps)$ for adaptive algorithms \cite{BCPRS17} (with a logarithmic
  advantage). Both algorithms work for
  real-valued functions %over $[n]^d$ and when the domain is restricted to the Boolean hypercube,
  %they
  and are shown to be optimal for real-valued functions  in \cite{BCPRS17}.

On the lower bound side, \cite{BMPR16} was the first to give a lower bound on testing unateness by showing that any non-adaptive algorithm with one-sided error must make $\Omega(\sqrt{n}/\eps)$ many queries. Then, \cite{CWX17} showed that unateness testing of Boolean functions
  requires $\widetilde{\Omega}(n^{2/3})$ queries for adaptive algorithms with two-sided error, showing that a polynomial gap between testing monotonicity and unateness for Boolean functions.\footnote{The conference version of the paper included a weaker lower bound of $\widetilde{\Omega}(\sqrt{n})$ for testing unateness. Since then, the authors have improved the lower bound to $\widetilde{\Omega}(n^{2/3})$ and have updated the full-version of the paper, available as \texttt{arXiv:1702.06997}.} For non-adaptive algorithms with one-sided error, \cite{CWX17, BCPRS17b} show $\widetilde{\Omega}(n)$ queries are necessary (for some constant $\eps>0$), which shows the~\mbox{algorithm} of \cite{CS16b,BCPRS17} is optimal among non-adaptive algorithms with one-sided error for Boolean functions. \vspace{-0.28cm}
%is optimal (up to polylogarithmic factors) by the upper bounds in \cite{CS16b, BCPRS17}.

\paragraph{Our Contribution.}  Generally, the power of adaptivity in property testing of Boolean functions
  is not yet well understood. %, despite being a natural and important question.
Taking the examples of monotonicity and unateness,
  the current best algorithms are both non-adaptive\hspace{0.03cm}\footnote{For real-valued functions,
  \cite{BCPRS17} showed that adaptivity helps by a logarithmic factor.} (ignoring polylogarithmic factors),
  and polynomial gaps remain between the best upper and lower bounds for the query complexity of adaptive algorithms.

%Even for the classic property of monotonicity, we cannot yet answer whether adaptive algorithms are strictly more powerful that non-adaptive algorithms. In fact, the current best monotonicity tester of \cite{KMS15} using $\widetilde{O}(\sqrt{n}/\eps^2)$ is non-adaptive; while the best adaptive lower bounds are of $\widetilde{\Omega}(n^{1/3})$ \cite{CWX17}.\footnote{Recently \cite{STW15}, showed that adaptive algorithms are strictly for powerful than non-adaptive algorithms for testing the class of Boolean juntas.}

%A very compelling question is whether adaptivity helps for unateness testing of Boolean functions---  can adaptive algorithms go below the \cite{CWX17} $\widetilde{\Omega}(n)$-query lower bound for non-adaptive, one-sided algorithms?

The main result of this work is an $\smash{\widetilde{O}(n^{3/4}/\eps^2)}$-query adaptive, one-sided algorithm for unateness
  testing of Boolean functions.

\begin{theorem}[Main]
\label{thm:main}
There is an $\widetilde{O}(n^{3/4}/\eps^2)$-query\hspace{0.01cm},\footnote{See (\ref{hehewiwi}) for the hidden
  polylogarithmic factor; we have made no effort to optimize the polynomial dependence on $\log n$ and $\log(1/\eps)$ in the algorithm.} adaptive algorithm
  with the following property: Given an %\vspace{-0.08cm}
$\eps>0$ and query access
to an unknown $f\colon \{0,1\}^n \to \{0,1\}$,
  it always returns ``unate''~if~$f$ is unate and % and \vspace{-0.17cm}
  returns ``non-unate'' with probability at least $2/3$ if $f$ is $\eps$-far from unate.
  % then the algorithm outputs ``non-unate'' with probability at least $2/3$.
%\end{itemize}
\end{theorem}

Compared to the $\widetilde{\Omega}(n)$ lower bound for non-adaptive, one-sided algorithms~\cite{CWX17}, Theorem~\ref{thm:main} implies that adaptivity helps by a polynomial factor for one-sided algorithms.
Additionally, given the lower bound of $\Omega(n/\eps)$ for unateness testing of real-valued functions
  over $\{0,1\}^n$ \cite{BCPRS17},~our result shows that Boolean functions are polynomially easier to test than real-valued functions. The current known upper and lower bounds for testing unateness for $\eps = \Theta(1)$ are summarized in the Table~1. 
  
\begin{table}\label{tab:current}
\centering
\begin{tabular}{|c||c|c|}
\hline
 & Adaptive & Non-adaptive \\
 \hline \hline
 Upper bounds & $\widetilde{O}(n^{3/4})$ (this work) & $O(n)$ \cite{BCPRS17}\\
 \hline
 Lower bounds & $\widetilde{\Omega}(n^{2/3})$ \cite{CWX17} & $\widetilde{\Omega}(n)$ (one-sided) \cite{CWX17, BCPRS17b} \\
 \hline
\end{tabular}
\caption{Current knowledge on upper and lower bounds for testing unateness. We consider the regime where $\eps = \Theta(1)$.}
\end{table}

Our algorithm is heavily inspired by the work of \cite{KMS15}, where they
  prove a  directed analogue of an isoperimetric inequality of Talagrand \cite{T93}
  and used it to reveal strong connections between the structure of
  anti-monotone edges of a Boolean function and its distance to monotonicity.~In~particular, their inequality implies that when~$f$~is~far from monotone, there must exist
  a  highly regular bipartite graph of certain size that consists of anti-monotone edges of $f$ only (see Theorem \ref{thm:kms}).
The analysis of~our~algorithm relies on this implication. (See more discussion later in
  Section \ref{sketchsec}.)

A recent work of \cite{CG17} introduced the notion of
  ``\emph{rounds}'' of adaptivity to quantify the degree of adaptivity used by a property testing algorithm.
We notice that our algorithm can be implemented using only two rounds of adaptivity.\vspace{-0.1cm}

\subsection{Binary search versus adaptive edge search\vspace{-0.05cm}}\label{sketchsec}

We give some high-level ideas behind our main algorithm.
First, it outputs ``non-unate'' only when an edge violation is found and thus,
  it is one-sided. Our analysis focuses on showing that, given
  a function that is $\eps$-far from unate, the algorithm finds an edge violation with high probability.

An edge violation occurs when two bi-chromatic edges \emph{collide}, i.e. they are in the same direction $i$ but one is monotone~and~the~other is anti-monotone. 
Thus, an algorithm may proceed by designing a subroutine for finding bi-chromatic edges and invoking this subroutine multiple times in hopes of finding a collision.
A subroutine for finding bi-chromatic edges that has been~widely~used~in~the~Boolean function property testing literature
  (e.g., \cite{B09, BB16,KS16})
  is \emph{binary search} (see Figure~\ref{fig:bs}):
%The underlying idea behind \cite{KS16} is to 1) determine whether influential directions are monotone or anti-monotone by finding a bi-chromatic edges, and 2) run a monotonicity tester on these influential directions after flipping anti-monotone coordinates. The first (and most interesting) step adopts a \emph{binary search strategy} to find bichromatic edges (see Figure~\ref{fig:bs}): \footnote{We note that a similar procedure was adopted in \cite{BB16} to give an algorithm which tests whether regular LTFs are monotone or $\eps$-far from monotone.}
\begin{enumerate}
\item Find two points $x, y \in \{0,1\}^n$
   with $f(x) \neq f(y)$, and let $S = \{ i \in [n] : x_i \neq y_i \}$. \vspace{-0.12 cm}
\item Pick a subset $S' \subset S$ of size $|S| / 2$,
  let $z = x^{(S')}$,\footnote{Here $x^{(S')} \in \{0, 1\}^n$ is the point obtained from $x$ by flipping its coordinates in $S'$;
  we also write $x^{(i)}$ for $x^{(\{i\})}$.} and query $f(z)$.\vspace{-0.12cm}
\item If $f(z) = f(x)$, let $x \leftarrow z$; if $f(z) = f(y)$, let $y \leftarrow z$. Repeat until
  $(x,y)$ is an edge.
\end{enumerate}
Clearly, the above procedure, if initiated with $f(x) \neq f(y)$,
  will always find a bi-chromatic edge~in some direction $i\in S$ with $O(\log n)$ queries.
One can further \emph{randomize} the subroutine by drawing $x$ and $y$ uniformly at random at the beginning
  %$(and continue when $f(x)\ne f(y)$)
  and drawing $S'$ uniformly at random from $S$ in~each round.
Given an $f$, the binary search subroutine naturally induces a distribution
  over bi-chromatic edges of $f$.
%,~e.g., let $p_i$ (or $q_i$) be the probability it finds~a~monotone (or anti-monotone) edge in direction $i$.
%An interesting question is:
%can we control the distribution over outputs when binary search is initiated under random points, and $S'$ is picked as a random subset? For instance,
%given an $f$ that is $\eps$-far from unate,
A high-level question is: Can we analyze
  this distribution for functions $f$ that are $\eps$-far from unate?
   Can this strategy give better algorithms for finding an edge violation?
%above binary search strategy output two edges in direction $i$, one of which is monotone, and the other is anti-monotone, with few queries?

\begin{figure}
\centering
\begin{picture}(230,230)
    \put(0,0){\includegraphics[width=0.5\linewidth]{images/binary-search.pdf}}
    \put(103, 115){$z$}
    \put(85, 150){$y$}
    \put(130, 74){$x$}
  \end{picture}
\caption{Pictorial representation of one step of the binary search strategy for finding bi-chromatic edges. The hypercube $\{0, 1\}^n$ is represented as the diamond. Points $x$ and $y$ are given with $f(x) = 0$ and  $f(y) = 1$ and a particular path represents flipping variables in $S$ one at a time. Finally $z = x^{(S')}$ corresponds to picking some $z$ between $x$ and $y$; in this case, $f(z) = 1$, so $y$ would be updated to $z$.}
\label{fig:bs}
\end{figure}

While we do not analyze the specific binary search strategy above in this paper, we introduce~a new kind~of edge search strategy, which we call \emph{adaptive edge search} and denote by $\ESearch$.~It is a crucial component~of our algorithm and allows for a relatively straightforward analysis. It~takes two inputs, a point $x\in \{0,1\}^n$
  and a nonempty set $S\subseteq [n]$,\hspace{0.01cm}\footnote{It is not important for the moment but later we will always   choose the size of $|S|$ to be smaller than $\sqrt{n}$.} with the goal of finding a bi-chromatic edge $(x,x^{(i)})$ for some $i\in S$
    (using $O(\log n)$ queries only).
The subroutine proceeds as follows:
\begin{enumerate}
%\item We start with some $x \in \{0, 1\}^n$ and $S \subset [n]$ where $x$ has a bi-chromatic edge in some direction $i \in S$.
\item Sample $L = O(\log n)$ subsets $T_1, \dots, T_L \subset S$ of size $|S| / 2$ uniformly, and query $f(x^{(T_\ell)})$.\vspace{-0.1cm}
\item Consider all $T_\ell$'s with $f(x^{(T_\ell)}) \neq f(x)$. If the intersection of such $T_\ell$'s consists of exactly \\one index $i\in S$, query $f(x^{(i)})$ and output $i$ if $f(x^{(i)})\ne f(x)$ (meaning that a bi-chromatic\\ edge
  $(x,x^{(i)})$ along direction $i$ has been found); otherwise return ``fail.''\end{enumerate}
See Figure \ref{fig:adaptive-esearch} for a pictorial representation.
While $\ESearch$ does not always finds~a bi-chromatic edge (unlike the binary search),
  its behavior is much easier to analyze.
Informally when $(x,x^{(i)})$ is a bi-chromatic edge  and $i\in S$ (otherwise it can never return $i$),
  $\ESearch(x,S)$ returns $i$ with high probability if
% with a set of sufficient conditions under which the
%  subroutine finds a bi-chromatic edge $(x,x^{(i)})$ along direction $i$ with high probability:
 % (1) $f(x)\ne f(x^{(i)})$ (otherwise it never returns $i$);
  (1)
%Consider the~case when $(x,x^{(i)})$ is a bi-chromatic~edge; otherwise it can never return $i$.%A sufficient condition for the subroutine to return $i$ with high~probability is that
  \emph{most} subsets $T\subset S$ of size $|S|/2$ with $i\notin T$
  have $f(x^{(T)})=f(x)$ and (2) \emph{most} $T\subset S$ of size~$|S|/2$ with $i\in T$
  have $f(x^{(T)})=f(x^{(i)})\ne f(x)$.
 (See Figure \ref{fig:adaptive-esearch} for an illustration.)

%With (1) and (2), one can show that with~high probability all $T_\ell$ sampled with $f(x^{(T_\ell)})\ne f(x)$
%  contain $i$ and no $j\ne i$ is contained in all such $T_\ell$; thus, the adaptive edge search returns $i$
%  and finds a (hidden) bi-chromatic edge $(x,x^{(i)})$ in direction $i$.

With the adaptive edge search in hand,
  the proof of Theorem \ref{thm:main}  proceeds in two steps.
For~the first step, we show that when $f$ is far from unate,  there must be
  ``many'' bi-chromatic edges $(x,x^{(i)})$ such that running $\ESearch$
  on $x$ paired with a random subset $S\subset [n]$ \emph{containing} $i$
  would lead to the discovery of  $(x,x^{(i)})$ with high probability.
There~are a lot of technical details hidden in the word ``many'': (i) subsets $S$ of different size
  contribute differently (intuitively, the larger~$S$, it is more likely for $S$ to
  contain $i$ when  $S$ is drawn from $[n]$ uniformly at random);
  (ii) we need~to balance the contribution from monotone and anti-monotone edges
  in the same direction  by taking their minimum. Intuitively, it will not help us find an edge violation
  if $\ESearch$ works well over many bi-chromatic edges in a direction $i$, but all these edges turn out to be
   monotone.~Following~the high-level discussion above,
  we formally introduce the notion of $\score^+_i$ and $\score^-_i $ for~a~Boolean
  function in Section \ref{sec:scores} (to measure the performance of $\ESearch$), and prove in Section \ref{sec:main2} that
\begin{align}\label{eqeqeq}
\sum_{i\in [n]} \min\big\{\score_i^+,\score_i^-\big\}=\widetilde{\Omega}(\eps^2),
\end{align}
when $f$ is $\eps$-far from unate. The proof of (\ref{eqeqeq}) heavily relies on the
   directed isoperimetric inequality~of \cite{KMS15} and its combinatorial implications for functions far
   from monotone
   (see Theorem \ref{thm:kms}).

In the second step, we present an algorithm that keeps calling the adaptive edge search (strategically),
  and show that it finds an edge violation with high probability, given (\ref{eqeqeq}).
%We will show that for functions which are $\eps$-far from unate, the above procedure (initialized to the proper parameters) can guess the correct direction $i \in S$ for many points $x$ where $(x, x^{(i)})$ is a bi-chromatic edge. Our algorithm will proceed by running the adaptive edge strategy (while modifying parameters) to look for an edge violation. See Figure~\ref{fig:adaptive-esearch} for a pictorial representation of the adaptive edge search strategy.
%Our main structural result about $\eps$-far-from-unate functions, stated in Lemma~\ref{main2} and proved in Section~\ref{sec:main2}, relies heavily on \cite{KMS15}. In fact, Lemma~\ref{main2} can be interpreted as a non-trivial connection between the directed isoperimetric theorems of \cite{KMS15} and the success of adaptive edge search strategy.
%Our algorithm based on (\ref{eqeqeq}) relies on the structure of
%  $f$ revealed by (\ref{eqeqeq}). %and its analysis ... blablabla
At a high level,~it starts by sampling a set $S\subset [n]$ of certain size and a sequence of
  $K_+$ points $\{x_i\}$ from $\{0,1\}^n$.~Then it runs $\ESearch(x_i,S)$ for each $x_i$ and keeps the directions of monotone edges found in a set~$A$.
Next it samples $M$ subsets $T_i\subseteq S$ of certain size and for each $T_i$,  it
  samples $K_-$ points $\{y_{i,j}\}$ to run $\ESearch(y_{i,j},T_i)$. Similarly, it keeps the directions of anti-monotone edges found in $B$.
Finally, it outputs ``non-unate'' if $A\cap B\ne \emptyset$, i.e., an edge violation is found; otherwise, it outputs ``unate''.

The tricky part is the choices of the size of sets $S$ and $T$ and the three  parameters
  $M,K_+$ and $K_-$.
For technical reasons, our algorithm is split into two cases, depending on how the $\widetilde{\Omega}(\eps^2)$
  in (\ref{eqeqeq}) is achieved, e.g., what scale of $\min\{\score_i^-,\score_i^+\}$
  contributes the most in the sum.~The parameters are chosen differently in the cases and their proofs use slightly different
  techniques. \vspace{-0.25cm}

\paragraph{Organization.} \hspace{-0.2cm}We formally introduce the adaptive edge search subroutine in Section~\ref{sec:aes}. Next,~we introduce the notion of scores and state (\ref{eqeqeq}) in Lemma~\ref{main2} in Section~\ref{sec:scores}. We present the algorithm and its analysis in
  Section~\ref{sec:algorithm}, assuming Lemma~\ref{main2}. Finally we prove Lemma~\ref{main2} in Section~\ref{sec:main2}.

\begin{figure}[t!]
\centering
\begin{picture}(275,275)
    \put(0,0){\includegraphics[width=0.6\linewidth]{images/adaptive-esearch.pdf}}
    \put(90, 85){$x$}
    \put(170, 98){$x^{(i)}$}
    \put(167, 187){$x^{(S)}$}
    \put(164, 145){$x^{(T_\ell)}$'s}
    \put(84, 127){$x^{(T_\ell)}$'s}
    \put(88, 175){$x^{(S\setminus \{i\})}$}
  \end{picture}
\caption{Pictorial representation of the adaptive edge search strategy, $\ESearch(x,S)$, for~finding bi-chromatic edges.
We consider the case when $(x,x^{(i)})$ is a bi-chromatic edge in direction~$i$~with $f(x)=0$ and $i\in S$.
%The hypercube $\{0, 1\}^n$ is represented with
The two sub-cubes in the picture above correspond to points that agree with $x$ outside of $S\setminus \{i\}$, and points that agree with
  $x^{(i)}$ outside of $S\setminus \{i\}$, respectively.
%restrictions to points agreeing in $x$ outside of coordinates in $S$. A possible $x$ with $f(x) = 0$ has a bi-chromatic edge in the $i$th direction.
The points~$x^{(T_\ell)}$ sampled in $\ESearch(x,S)$
%are in their restricted hypercubes
  lie in one of the sub-cubes according to whether $i \in T_{\ell}$ or not. % (points on the left restricted sub-cube have $i \notin T_{\ell}$, and points in the right restricted sub-cube have $i \in T_{\ell}$).
%$\ESearch(x,S)$ returns $i$ if all $x^{(T_\ell)}$
Under certain conditions one can show that with high probability, all $T_\ell$'s with $f(x^{(T_\ell)})=1$~lie in~the~right sub-cube and furthermore, their intersection is exactly $\{ i \}$.
In this case, $\ESearch$ returns $i$.}
\label{fig:adaptive-esearch}
\end{figure}


==> temp - Erik/scores-lemma.tex <==
% !TEX root =  writeup.tex

\section{Proof of Lemma \ref{main2}}\label{sec:main2}

We first show that Lemma \ref{main2} follows from the following lemma that we prove in this section.

\begin{lemma}\label{main4}
If $f\colon\{0,1\}^n\rightarrow \{0,1\}$ is $\eps$-far from unate and $I_f \leq 6\sqrt{n}$,
  then we have
\begin{equation}\label{maineq4}
\sum_{i=1}^n \score_i^- \geq \Omega\left(\dfrac{\eps^2}{\log^8 n}\right).
\end{equation}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{main2} assuming Lemma \ref{main4}]
Suppose that the LHS of (\ref{maineq}) is achieved by
$$
\sum_{i\in W}\score_i^+ +\sum_{i\notin W} \score_i^-
$$
for some $W\subseteq [n]$.
Then we let $r\in \{0,1\}^n$ be the string with $r_i=1$ if $i\in W$ and $r_i=0$ if $i\notin W$,
  and let $g$ be the Boolean function with $g(x)=f(x\oplus r)$.
On the one hand, $g$ has the same distance to unateness as $f$ and satisfies $I_g=I_f$,
  so Lemma \ref{main4} applies to $g$.
On the other hand, it follows from the description of $\ESearch$ and
  the definition of $\score$ that $\score_i^-$ of $g$ is exactly the same
  as $\score_i^+$ of $f$ if $i\in W$ or $\score_i^-$ of $f$ if $i\notin W$.
To see this is the case, note that the output distribution of $\ESearch(x,S)$ on $g$
  is exactly the same as that of $\ESearch(x\oplus r,S)$ on $f$.
As a result, whether $(x,S)$ is a good pair
  or not in $g$ is the same as that of $(x\oplus r,S)$ in $f$ (except that the roles of $E_i^+$ and $E_i^-$
  may get switched depending on whether $i\in W$ or not).
(\ref{maineq}) for $f$ then follows from (\ref{maineq4}) for $g$.
\end{proof}

We prove Lemma \ref{main4} in the rest of the section.
Let $f$ be a function that is $\eps$-far from unate and has $I_f = O(\sqrt{n})$.
Let $G_f$ be the bipartite graph of \emph{anti-monotone edges} of $f$ defined as follows:
\begin{flushleft}\begin{enumerate}
\item Vertices on the LHS of $G_f$ correspond to points $x\in \{0,1\}^n$ with $f(x)=1$ and vertices
  on the RHS of $G_f$ correspond to points $y\in \{0,1\}^n$ with $f(y)=0$;
\item $(x,y)$ is an edge in $G_f$ if $(x,y)$ is an anti-monotone edge.
\end{enumerate}\end{flushleft}
We recall a key technical lemma from \cite{KMS15} which states that when $f$ is $\eps$-far from
  monotone (which is the case here since $f$ is $\eps$-far from unate), $G_f$ must contain a large and ``good'' subgraph.

\begin{definition}
Let $G=(U,V,E)$ be a bipartite subgraph of $G_f$, where $U$ is a set of points $x$ with $f(x)=1$, $V$ is a set of points $y$ with $f(y)=0$, and $E$ consists
  of anti-monotone edges of $f$.
We say $G$ is right-$d$-good, for some positive integer $d$, if the degree of every $y\in V$ is in the range $[d,2d]$ and
  the degree of every $x\in U$ is at most $2d$, and $G$ is left-$d$-good if the degree
  of every $x\in U$ is in the range $[d,2d]$ and the degree of every $y\in V$ is at most $2d$.
\end{definition}

%Since $f$ is $\eps$-far from unateness and thus,
%  $\eps$-far from monotone we have the following lemma from \cite{KMS}:
%  know from [KMS] that there exist a bipartite graph $G$ between
%  $U$ and $V$ such that (we assume below that $U$ has degree between $d$ and $2d$ and $V$ has degree
%  at most $2d$ but the other case is symmetric). Thus, our starting point is the following theorem:
\begin{theorem}[Lemma 7.1 in \cite{KMS15}]
\label{thm:kms}
If $f$ is $\eps$-far from monotone, then $G_f$ contains a bipartite subgraph $G=(U,V,E)$
  that satisfies one of the following conditions:
%There exists a bipartite graph $G = (U, V, E)$ where $U, V \subset \{0, 1\}^n$, satisfying the three following properties:
\begin{enumerate}
%\item $f(x)=1$ for each $x\in U$ and $f(y)=0$ for each $y\in V$, and $(x, y) \in E$ is a anti-monotone edge in $f$.
%\item The degree of each vertex $x\in U$ is between $d$ and $2d$ for some parameter $d\ge 1$\\
%  and the degree of each vertex $y\in V$ is at most $2d$;
\item $G$ is left-$d$-good for some positive integer $d$ and
  $\sigma=|U|/2^n$ satisfies
\begin{equation}\label{hehehehe}
\sigma^2 d= \Theta\left(\frac{\eps^2}{\log^4 n}\right).
\end{equation}
\item $G$ is right-$d$-good for some positive integer $d$ and
  $\sigma=|V|/2^n$ satisfies (\ref{hehehehe}).
\end{enumerate}
\end{theorem}

Since $f$ is $\eps$-far from unate and in particular, $\eps$-far from monotone,
  Theorem \ref{thm:kms} applies to $f$ and we use $G=(U,V,E)$ to denote such a subgraph of $G_f$.
In the rest of the proof we assume without loss of generality that
  $G$ is left-$d$-good and $\sigma=|U|/2^n$ satisfies (\ref{hehehehe});
  the proof for the other case when $G$ is right-$d$-good is symmetric.
%For convenience, consider a subgraph of $G$ where $\sigma^2 d = \Theta(\frac{\eps^2}{\log^4 n})$ by removing nodes and edges.
Given $G$ and $\sigma$, we choose the $t$ to be the largest integer with
\begin{equation}\label{choiceoft}
2^{t-1}\le \left\lceil \frac{\sigma\sqrt{n}}{\log^4 n} \right\rceil.
\end{equation}
So we have $t\ge 1$. Using $\sigma\le 1$, we also have $t< \Lambda$ and thus, $t\in [\Lambda]$.
%(\ref{hehehehe}), we have
%$$
%\frac{\sigma\sqrt{n}}{\log^4 n}=\Theta\left(\frac{\eps}{\log^6 n}\cdot \sqrt{\frac{n}{d}}\right)
%\le O\left(\frac{\sqrt{n}}{{\log^6 n}}\right)<\Lambda
%$$
%and thus, $t\in [\Lambda]$.
% $\sigma \sqrt{n} \leq \frac{n}{d}$ since otherwise, $\sigma \geq \frac{\sqrt{n}}{d}$ and then $\sigma^2 d \geq \frac{n}{d} > 1$, but $\sigma^2 d = O(\frac{1}{\log^4 n})$.

Our goal is to show the following lemma from which Lemma \ref{main4} follows directly:
\begin{lemma}\label{main3}
Let $G = (U, V, E)$ be a subgraph of $G_f$ that is left-$d$-good and satisfies (\ref{hehehehe}).
% satisfying the conditions of Theorem~\ref{thm:kms}, and $2^t = \Theta(\frac{\sigma \sqrt{n}}{\log^4 n})$, then
Then 
\begin{equation} \dfrac{2^t}{\sqrt{n}}\cdot \sum_{i=1}^n \score_{i, t}^{-} = \Omega\left(\dfrac{\eps^2}{\log^8 n}\right) . \label{eq:maineq22}
\end{equation}
\end{lemma}
%The above lemma would imply Lemma~\ref{main2} by considering all possible orientations, and noting that Theorem~\ref{thm:kms} will provide one such graph $G$ for each orientation, since we assume our original function is $\eps$-far from unate.

To gain some intuition, assume
  that every $(x,y)\in E$ in direction $i$ has $x$ being $t$-strong for $E_i^-$ (we always use
  $x$ to denote points in $U$ and $y$ or $x^{(i)}$ to denote points in $V$ in the rest of the proof). Then, each edge
  in $E$ contributes ${1}/{2^n}$ to the sum on the LHS of (\ref{eq:maineq22}) and thus,
  it is at least
\begin{equation}
\frac{2^t}{\sqrt{n}}\cdot \frac{|E|}{2^n}\ge \frac{2^t}{\sqrt{n}}\cdot \frac{d|U|}{2^n}=
\dfrac{2^t}{\sqrt{n}} \cdot \sigma d = \Omega\left( \dfrac{\sigma \sqrt{n}}{\log^4 n \cdot \sqrt{n}} \right) \cdot \sigma d = \Omega\left( \dfrac{\sigma^2 d}{\log^4 n} \right) = \Omega\left(\dfrac{\eps^2}{\log^8 n} \right),\label{eq:deduce}
\end{equation}
where the first inequality follows from the fact that $G$ is left-$d$-good
  and the last equation uses (\ref{hehehehe}). Note that for the specific case when $t=1$, every edge $(x, y) \in E$ in direction $i$ is $t$-strong for $E_i^{-}$; thus, this intuition holds formally, and we may assume for the rest of the proof that $t > 1$.

The plan for the rest of the proof is as follows. First we give
  a sufficient condition for a point $x\in U$ to be $t$-strong for $E_i^-$.
Next, we prove a persistency lemma similar to that from \cite{KMS15} to show that for
  most edges $(x,x^{(i)})\in E$, $x$ is $t$-strong
  for $E_i^-$. %if $(x,y)$ is along direction $i$.
Finally, by a similar argument to (\ref{eq:deduce}), we obtain the same conclusion only losing only a constant factor in the inequality.

More specifically, in Section~\ref{sec:robust} we define the notion of \emph{robust} sets, and show that if an edge
  $(x,x^{(i)})\in E$
has many robust sets, its left endpoint $x$ is $t$-strong for $E_i^-$.
Then in Section~\ref{sec:solid}, we introduce the notion of \emph{solid} edges, %which is attained through the notion of persistence,
  and show that 1) most edges of $E$ are solid and 2) every {solid} edge have many robust sets, which then finishes the proof.%The schema is:
%\[  E \to \text{solid edges} \to \text{edges with many robust sets} \to \text{$t$-strong endpoints}.\]
%The next subsection corresponds to the last arrow, and the following to the first two arrows.

\subsection{Edges with many robust sets have strong left endpoints}\label{sec:robust}

We now introduce the notion of robust sets $S\in \calP_{i,t}$ for anti-monotone edges $(x,x^{(i)})\in E$
  (with $x\in U$ being the left endpoint and $i$ being the direction).
%This notion allows us to relate bichromatic edges with $t$-strong points.
Intuitively, we would like to show that if
  $S\in \calP_{i,t}$ is a robust set for $(x,x^{(i)})$,
  then $\ESearch(x, S \cup \{ i \})$ returns $i$ with probability at least $\frac{1}{2}$ and thus,
  $(x,S)$ is a good pair for $E_i^-$.
This is shown in Lemma \ref{lem:robust}.
As a result, to show that $x$ is $t$-strong for $E_i^-$, it suffices to show
  that most sets $S\in \calP_{i,t}$ are robust for $(x,x^{(i)})$.
%an edge $(x, x^{(i)})$ has many robust sets, then $x$ is $t$-strong for $E_i^-$, i.e., $\ESearch(x, S \cup \{ i \})$ succeeds for many sets $S \in \calP_{i, t}$.

\begin{definition}[Robust Sets]\label{def:robust}
Let $(x, x^{(i)})\in E$. % be a bichromatic edge of $G$ and consider $S \in \calP_{i, t}$.
We say $S\in \calP_{i,t}$ is a \emph{robust} set for $(x, x^{(i)})$ if:
\begin{enumerate}
\item At least $(1 - ( {1}/{\log^2 n}))$-fraction of subsets $S' \subset S$ of size $2^{t-1} - 1$ has $f(x^{(S' \cup \{ i \})}) \neq f(x)$.\vspace{-0.1cm}
\item At least $(1 - ( {1}/{\log^2 n}))$-fraction of subsets $S' \subset S$ of size $2^{t-1}$ has $f(x^{(S')}) = f(x)$.
\end{enumerate}
Note that for the special case when $t=1$ (letting $S=\{j\}$ for some $j\ne i$),
  conditions 2 and 3 above require
  $f(x^{(i)})\ne f(x)$ and $f(x^{(j)})=f(x)$, respectively.
\end{definition}

We show that if $S\in \calP_{i,t}$ is robust for an edge $(x,x^{(i)})\in E$, then
  $(x,S)$ is a good pair for $E_i^-$.

\begin{lemma}\label{lem:robust}
If $S\in \calP_{i,t}$ is a robust set for $(x,x^{(i)})\in E$, then $\ESearch(x, S\cup\{i\})$
  returns $i$ with high probability (and thus, $(x,S)$ is a good pair for $E_i^-$).
\end{lemma}
\begin{proof}
Let $S\in \calP_{i,t}$ be a robust set for $(x,x^{(i)})\in E$.
The proof consists of two claims.
%Combining both claims one concludes that with probability at least $\frac{3}{4}$, the set $C$ from line $8$ of $\ESearch$ will be equal to $\{ i \}$, which gets the desired outcome.
The first claim shows that in $\ESearch(x,S\cup\{i\})$,
  we have $i\in C$ at the end of Step 3 with high probability.
The second claim shows that $C$ does not contain any $\ell\in S$ with high probability.

%We start with the first claim:

\begin{claim}
With probability at least $1 - o(1)$, we have $i \in \bC$ in Step $3$ of $\ESearch(x,S\cup \{i\})$.
\end{claim}
\begin{proof}
We use $\bT_1, \ldots, \bT_L$ to denote the $L$ random subsets sampled in Step 3 of $\ESearch$.
For $i\notin \bC$ to happen, either every $\bT_\ell$ satisfies $f(x^{(\bT_\ell)})=f(x)$,
  or one of the $\bT_\ell$ satisfies $f(x^{(\bT_\ell)})\ne f(x)$
  and $i\notin \bT_\ell$. %, or every $T_\ell$ that with $f(x^{(T_\ell)})\ne f(x)$.
Below we upperbound the probability of each of these two events by $o(1)$.
The claim then follows by a union bound on the two events.

First, by condition 1 of Definition \ref{def:robust},
  the probability of $f(x^{(\bT_\ell)})\ne f(x)$ for each $\ell$ is at least (by only considering the case when $i\in \bT_\ell$)
$$
(1/2)\cdot (1-(1/\log^2 n))
$$
and thus, the probability of the first event is $o(1)$ using our choice of $L=\lceil 4\log n\rceil$.

%Second, the probability that $i\notin T_k$ for all $k\in[L]$ is at most $1/2^L$. If there is some $k\in[L]$ such that $i\in T_k$, then following the second statement from definition of robust sets we know with probability at most $1/\log^2 n$ we have $f(x^{(T_k)}) = f(x)$. Therefore with probability at least $1-1/2^L-1/\log^2 n$ there exists $k\in[L]$ such that $i\in T_k$ and $f(x^{(T_k)}) \not= f(x)$.

Next by condition 2 of Definition \ref{def:robust},
  the probability of $i\notin \bT_\ell$ and $f(x^{(\bT_\ell)})\ne f(x)$ is at most
$$
(1/2)\cdot (1/\log^2 n)=1/(2\log^2 n).
$$
%, for some $k\in[L]$ if $T_k$ is any set with $i\notin T_k$, then $T_k\subset S$ has size $2^{t-1}$, and following the third statement from definition of robust sets we know the probability that $f(x^{(T_k)}) \not= f(x)$ is at most $\frac{1}{\log^2 n}$.
By a union bound on $\ell \in [L]$ and our choice of $L$,
  the probability of the second event is also $o(1)$.
%   we know the probability that there exists $k\in[L]$ such that $i\notin T_k$ and $f(x^{(T_k)}) \not= f(x)$ is at most $\frac{L}{\log^2 n}=\frac{1}{\log n}$.
%Combining the two arguments above we know with probability at least $1 - \frac{1}{\log n}$ we have $i \in C$ at line $8$.
\end{proof}
%First, consider the sets $T_k$ sampled in line $7$ where $i \in T_k$. Then with probability at least $1 - \frac{K}{\log^2 n} - \frac{1}{2^{K}}$, there is at least one such set, and all $T_k \setminus \{i \}$ are subsets of size $2^t - 1$ where $f(x^{(T_k)}) \neq f(x)$. Second, if $T_k$ is any set sample with $i \notin T_k$, then $T_k \subset S$ of size $2^{t-1}$, so with probability $1 - \frac{1}{\log^2 n}$, $f(x^{(T_k)}) = f(x)$, so we union bound over at most $K$ such sets. Thus, $i \in C$ with probability at least $1 - O(\frac{1}{\log n})$.

\begin{claim}
With probability at least $1-o(1)$, we have $\bC \cap S=\emptyset$ in Step 3 of $\ESearch(x,S\cup\{i\})$.
% $l \in S$, then $l \notin C$
\end{claim}
\begin{proof}
Consider an index $k \in S$ and note that $k \neq i$. Then, in order to have $k\in \bC$,
  none of the $\bT_\ell$ can satisfy both $f(x^{(\bT_\ell)})\ne f(x)$ and $k\notin \bT_\ell$.
However,
%, there must exists a set sampled $T_k \subset S \cup \{ i \}$ in line 6 where $f(x^{(T_k)}) \neq f(x)$ and $l \notin T_k$.
there are $\smash{\binom{2^t-2}{2^{t-1} - 1}}$ subsets of $S \cup \{ i\}$ of size $2^{t-1}$ which include $i$ and exclude $k$. Among them the number of $T$ with $f(x^{(T)})=f(x)$ is at most $$\frac{1}{\log^2 n} \cdot \binom{2^{t} - 1}{2^{t-1} - 1}$$
by condition 2. So the fraction of $T$ that includes $i$, excludes $k$, and has $f(x^{(T)})\ne f(x)$ is at least
\[\dfrac{\binom{2^t-2}{2^{t-1} - 1} - \frac{1}{\log^2 n} \cdot \binom{2^{t} - 1}{2^{t-1} - 1}}{\binom{2^t}{2^{t-1}}} \geq \frac{1}{4} - \frac{1}{2\log^2 n}=\frac{1}{4}-o(1). \]
Thus, the probability of $k \in \bC$ is at most $(3/4+o(1))^L$.
This is $o(1/n)$ by our choice of $L=\lceil 4\log n\rceil $.
The lemma then follows by a union bound over all $k\in S$.
%becomes very small if $L = c_1 \log n$ for a large enough $c_1$, and we may union bound over all $l \in S$ with $l \neq i$.
\end{proof}

It follows that $\bC=\{i\}$ with probability $1-o(1)$.
This finishes the proof of Lemma \ref{lem:robust}.
\end{proof}

\subsection{Solid edges have many robust sets}\label{sec:solid}

We now introduce the notion of $(\tau,\gamma)$-persistent.
These are points $x$ at which the value of $f$ remains the same as $f(x)$ with high probability (at least $1-\gamma$)
  after flipping $\tau$ random bits of $x$.

\begin{definition}[Persistent Points]
Let $\tau:0\le \tau\le n$ be a nonnegative integer and $\gamma\in [0,1]$.
We say a point $x\in \{0,1\}^n$ is
  $(\tau,\gamma)$-persistent in $f$ if, by flipping a set $\bS\subseteq [n]$ of size $\tau$ drawn uniformly at random, we have
  $\Pr_{\bS} [f(x)\ne f(x^{(\bS)}) ]\le \gamma.$
For the special case of $\tau=0$, every $x\in \{0,1\}^n$ is $(0,\gamma)$-persistent for all $\gamma\in [0,1]$.
\end{definition}
\begin{remark}
\begin{flushleft}For readers familiar with \emph{\cite{KMS15}},
  our definition of persistency is slightly different from that of \emph{\cite{KMS15}}: 1) we need the second parameter
  $\gamma$ while \emph{\cite{KMS15}} always sets $\gamma=1/10$;
  2) More importantly, \emph{\cite{KMS15}} only allows one to randomly flip $0$-entries of $x$ to $1$
  (since they are interested in monotonicity testing) while we flip all sets of $\tau$ coordinates
  of $x$ uniformly at random.
\end{flushleft}\end{remark}

We need the following persistency lemma. Its proof is similar to Lemma 9.3 of \cite{KMS15}.
Due to differences discussed above, we give a self-contained proof adapted from \cite{KMS15}
  in Appendix~\ref{persistency-proof}.

%Note that [KMS] is interested in flipping $\tau$ $0$'s to $1$'s; here, we
%  can flip any bits, which I think actually make the proof of the following lemma
%  from [KMS] slightly easier (in particular, they spent some effort to analyze
%  the distribution of $x^\ell$ but in our case it is simply the uniform distribution).

\begin{lemma}[Persistency lemma]\label{persistency-lemma}
For $\gamma\in(0,1]$ and $\tau\in[0,n]$, the fraction of $(\tau,\gamma)$-non-persistent points is 
  at most $O(I_f\cdot \tau/(n\gamma))$.
\end{lemma}

Let $\gamma=1/{\log^3 n}$. As $I_f=O(\sqrt{n})$, the fraction of $(\tau,\gamma)$-non-persistent
  points is at most $$O\left(\frac{\tau \cdot \log^3 n}{\sqrt{n}}\right).$$
Next we introduce the notion of \emph{solid} edges in $G$ and prove using the persistency lemma that
  most edges in $G$ are solid.

\begin{definition}[Solid Edges]
An edge $(x,y)$ in $G$ (with $x\in U$ and $y\in V$ as usual) is \emph{solid} if $x$ is $(2^{t-1},\gamma)$-persistent
  and $y$ is $(2^{t-1} - 1,\gamma)$-persistent.
\end{definition}

%We show that most edges in $G$ are solid.% and then for every solid edge $(x,y)$ with $y=x^{(i)}$.

\begin{lemma}\label{manysolid}
At least $(1-o(1))$-fraction of edges of $G$ are solid.
\end{lemma}
\begin{proof}
First recall that the number of edges in $G$ is $\Theta(\sigma 2^n\cdot d)$.
Using the persistency lemma,
  the fraction of points (with respect to the full set of size $2^n$)
  that are $(2^{t-1},\gamma)$-non-persistent is at most
\begin{equation}\label{hehehehehe}
O\left(\frac{2^{t-1} \cdot \log^3 n}{\sqrt{n}}\right). %= {2^t}\cdot O\left(\frac{\log^3 n}{\sqrt{n}}\right).
%O\left(\frac{\sigma\sqrt{n}}{\log^{4} n}\cdot \frac{\log^3 n}{\sqrt{n}}\right)=o\left(\sigma\right).
\end{equation}
By our choice of $t$ in (\ref{choiceoft}), and the fact that $t > 1$,
$\sigma\sqrt{n}/\log^4 n\ge 1$, in which case we have $2^{t-1}=O(\sigma\sqrt{n}/\log^4 n)$
  and (\ref{hehehehehe}) becomes $O(\sigma/\log n)=o(\sigma)$,

%(The latter follows from (\ref{hehehehehe}) since $d\le n$ and thus, $\sigma=\Omega(\eps/(\sqrt{n}\log^2 n))$.)
As a result, the number of edges $(x,y)$ in $G$ with $x$ being $(2^{t-1},\gamma)$-non-persistent
  is $o(\sigma 2^n\cdot d)$.
By a similar argument one can show that the number of edges $(x,y)$ in $G$ with $y$
  being either $(2^{t-1}-1,\gamma)$-non-persistent is
  $o(\sigma2^n \cdot d)$, at most a $o(1)$-fraction of edges in $G$.
%The number of inputs that are $(2^t, \gamma)$-non-persistent is also at most $o(\sigma)$, so taking a union bound, we remove at most
%$$
%o(\sigma \cdot d \cdot 2^n)
%$$
%many edges. All edges that remain are solid.
\end{proof}

%Let $(x,y)$ be a solid edge in $G$ with $y=x^{(i)}$, $i\in [n]$.
%We show that $(x, x^{(i)})$ has many robust sets, which completes the last step of the proof of Lemma~\ref{main3}.

Finally we show that every solid edge in $G$ has many robust sets in $\calP_{i,t}$.

\begin{lemma}\label{manyrobust}
Suppose that $(x, x^{(i)})\in E$ is a solid edge in $G$. Then the fraction of sets $S\in \calP_{i,t}$
  that are not robust with respect to edge $(x,x^{(i)})$ is at most ${4}/{\log n}.$
\end{lemma}

\begin{proof}
By definition, a set $S\in \calP_{i,t}$ is not robust for $(x,x^{(i)})$
  if one of the following events occur:
\begin{enumerate}
\item At least $(1/\log^2 n)$-fraction of subsets $T\subset S$ of size $2^{t-1} - 1$
  have $f(x^{(T \cup \{i \})}) = f(x)\ne f(x^{(i)})$.\vspace{-0.12cm}
\item At least $(1/\log^2 n)$-fraction of subsets $T\subset S$ of size $2^{{t-1}}$
  satisfy $f(x^{(T)}) \neq f(x)$.
\end{enumerate}
We bound the fraction of such $S$ in $\calP_{i,t}$ for each event separately.

For the second event, we consider the following bipartite graph $H'$.
Vertices $U'$ on the LHS of $H'$ correspond to subsets $T$ of $[n]\setminus \{i\}$ of size
  $2^{t-1}$; vertices on the RHS correspond to $S\in \calP_{i,t}$;
  $(T,S)$ is an edge iff $T\subset S$.
Clearly $H'$ is bi-regular. Let $d_{\text{left}}$ and $d_{\text{right}}$ denote the degrees.
%Let $U'$ be the set of vertices on the LHS.
Let $\alpha$ be the fraction of $S$ among $\calP_{i,t}$ (the RHS) for which the second event occurs.
Then the number of $T$ with $f(x^{(T)})\neq f(x)$ is at least
$$
\alpha \cdot |\calP_{i,t}|\cdot d_{\text{right}} \cdot \frac{1}{\log^2 n} \cdot\frac{1}{d_{\text{left}}}
=\alpha\cdot |U'| \cdot \frac{1}{\log^2 n} =\alpha \cdot \frac{1}{\log^2 n} \cdot \binom{n-1}{2^{t-1}}.
$$
However, as $x$ is $(2^{t-1},\gamma)$-persistent, the number of such $T$ is
  at most $
\gamma \cdot \binom{n}{2^{t-1}}.
$
As a result we have
$$
\alpha \le \log^2 n \cdot \gamma \cdot \frac{\binom{n}{2^{t-1}}}{\binom{n-1}{2^{t-1}}} \le \frac{2}{\log n}.
$$

For the first event, we consider a similar regular bipartite graph $H^*$. Vertices
  $U^*$ on the LHS correspond to subsets $T$ if $[n] \setminus \{ i \}$ of size $2^{t-1} -1$; vertices on the RHS correspond to $S \in \calP_{i,t}$; $(T,S)$ is an edge iff $T \subset S$. Similarly, we let $\beta$ be the fraction of $S$
    among $\calP_{i,t}$ (the RHS) for which the first event occurs. Then the number of $T$ with $f(x^{(T \cup \{ i \})}) =f(x)\ne f(x^{(i)})$ is at least
\[ \beta \cdot |\calP_{i,t}| \cdot d_{\text{right}} \cdot \dfrac{1}{\log^2 n} \cdot \frac{1}{d_\text{left}} = \beta \cdot |U^*| \cdot \dfrac{1}{\log^2 n} = \beta \cdot \frac{1}{\log^2 n} \cdot \binom{n - 1}{2^{t-1}-1}. \]
However, since $x^{(i)}$ is $(2^{t-1}-1, \gamma)$-persistent, the number of such $T$ is at most
$ \gamma \cdot \binom{n}{2^{t-1} - 1} $.
Thus,
\[ \beta \leq \log^2n \cdot \gamma\cdot \dfrac{ \binom{n}{2^{t-1}-1}}{\binom{n-1}{2^{t-1}-1}} \leq \frac{2}{\log n}. \]
So the total fraction of sets $S\in \calP_{i,t}$ that satisfy one of the events is at most ${4}/{\log n}$.
\end{proof}

\subsection{Finishing the proof of Lemma \ref{main3}}

From Lemma \ref{manysolid}, we know the number of solid edges in $G$ is at least $\Omega(|E|)$.
Combining Lemma \ref{manyrobust} with Lemma \ref{lem:robust}, we know for each solid edge $(x,x^{(i)})$ in $G$, at least $(1-4/\log n)$-fraction of sets in $\calP_{i,t}$ are robust, and its left end point
  $x$ is $t$-strong for $E_i^-$ and contributes $1/2^n$ to
  $\score_{i,t}^-$ in the LHS of (\ref{eq:maineq22}).
Lemma \ref{main3} then follows from the same analysis done in (\ref{eq:deduce}), after
  replacing $|E|$ by $\Omega(|E|)$ at the beginning.



